MACI: Multi-Agent Collaborative Intelligence for Adaptive Reasoning and Temporal Planning

Artificial intelligence requires deliberate reasoning, temporal awareness, and effective constraint management, capabilities traditional LLMs often lack due to their reliance on pattern matching, limited self-verification, and inconsistent constraint handling. We introduce Multi-Agent Collaborative Intelligence (MACI), a framework comprising three key components: 1) a meta-planner (MP) that identifies, formulates, and refines all roles and constraints of a task (e.g., wedding planning) while generating a dependency graph, with common-sense augmentation to ensure realistic and practical constraints; 2) a collection of agents to facilitate planning and address task-specific requirements; and 3) a run-time monitor that manages plan adjustments as needed. By decoupling planning from validation, maintaining minimal agent context, and integrating common-sense reasoning, MACI overcomes the aforementioned limitations and demonstrates robust performance in two scheduling problems.

==> AlternateView.tex <==
%\newpage
\section*{Required Statement: Alternative Approaches and MACI's Advantages}

Several alternative approaches have been proposed to address the limitations of LLM in planning tasks. These alternatives fall into three main categories: enhancing single-LLM architectures, implementing hybrid systems, and developing specialized tools.

\textbf{The single-LLM enhancement} approach proposes integrating memory modules, logical reasoning layers, and constraint-aware training to improve LLM capabilities. Although these enhancements could potentially address some limitations, they face a fundamental challenge: the ``average modelproblem ''. Training a single model to handle diverse planning domains inevitably leads to compromises that reduce effectiveness in specific tasks. Moreover, continually expanding the model to cover new domains creates unsustainable computational demands and risks degrading performance across all tasks.

\textbf{Hybrid approaches}, such as neuro-symbolic systems and retrieval-augmented generation (RAG), attempt to combine LLMs with external knowledge bases and reasoning modules. Although these approaches offer valuable capabilities, they typically implement rigid predetermined integration patterns that lack the flexibility needed for complex planning tasks. In addition, these systems often maintain centralized control structures that cannot overcome the attention-narrowing problems inherent in single-model architectures.

\textbf{Tool-based solutions} propose coupling LLMs with specialized software like optimization solvers and knowledge graphs. However, these solutions primarily augment rather than fundamentally transform LLM capabilities. The tools operate as black boxes, unable to participate in the kind of dynamic, multi-perspective reasoning required for robust planning.

MACI addresses these limitations through its meta-planning architecture and specialized agents. Unlike single-model enhancements, MACI's agents can maintain domain expertise without averaging effects. Unlike hybrid systems, MACI enables flexible and task-specific agent configurations. Unlike tool-based approaches, MACI agents actively participate in the planning process through structured collaboration and validation protocols.


==> ConclusionOld.tex <==

\section{Conclusions with Impact Statements}
\label{sec:MACIConc}

Current artificial intelligence systems excel at pattern matching but struggle with deliberate analytical reasoning required for complex planning. While Large Language Models (LLMs) demonstrate impressive capabilities, they face three critical limitations: inability to validate their own outputs (paralleling Gödel's incompleteness theorems), inconsistent maintenance of constraints during planning, and inadequate integration of common-sense knowledge. Our experiments demonstrate that existing multi-agent systems, focused primarily on coordination, fail to address these limitations.

MACI (Multi-Agent Collaborative Intelligence) advances the state of the art through three key contributions:

\begin{enumerate}[leftmargin=1.2em, topsep=-.15em, parsep=-.15em]
   \item \textbf{Meta-Planning Architecture:} MACI generates specialized planning workflows by:
       \begin{itemize}[leftmargin=1.0em, topsep=-.15em, parsep=-.15em]
           \item Constructing role-node and dependency networks.
           \item Identifying implicit constraints through common-sense analysis.
           \item Establishing validation across distributed agents.
       \end{itemize}
   
   \item \textbf{Workflow Enhancement:} As demonstrated in our experiments:
       \begin{itemize}[leftmargin=1.0em, topsep=-.15em, parsep=-.15em]
           \item Sequential Planning: Enhanced workflow $\mathbf{W^*}$ enabled all LLMs to generate feasible solutions.
           \item Reactive Planning: Early information agent in $\mathbf{W^R}$ enabled proactive replanning.
           \item Unexpected synergy: DeepSeek contributed spatial optimizations beyond MACI's specifications.
       \end{itemize}
   
   \item \textbf{Empirical Validation:} Our Thanksgiving dinner planning case study shows:
       \begin{itemize}[leftmargin=1.0em, topsep=-.15em, parsep=-.15em]
           \item Improving constraint satisfaction on LLMs.
           \item Effective handling of crises through early detection.
           \item Clear performance differences between LLMs in utilizing MACI's capabilities.
       \end{itemize}
\end{enumerate}

MACI demonstrates that addressing LLM limitations requires more than simple agent coordination. It demands a structured meta-planning architecture that enables comprehensive constraint awareness and validation. The framework's success in complex temporal planning, coupled with unexpected improvements from LLM contributions, suggests a promising direction for developing more capable AI planning systems.


==> EmergencyProcedure.tex <==
\begin{table*}[ht]
\caption{Dynamic Adjustment Procedures}
\footnotesize
\begin{tabular}{|p{0.2\textwidth}|p{0.25\textwidth}|p{0.25\textwidth}|p{0.2\textwidth}|}
\hline
\textbf{Event Type} & \textbf{Detection} & \textbf{Response} & \textbf{Validation} \\
\hline
Flight Delay &
Monitor: flight\_status() \newline
Threshold: delay > 30min &
1. Recalculate pickup time \newline
2. Reassign drivers \newline
3. Update dependencies &
Verify: \newline
- New schedule feasible \newline
- Resources available \\
\hline
Cooking Delay &
Monitor: cooking\_progress() \newline
Threshold: lag > 15min &
1. Adjust side dish schedule \newline
2. Reallocate supervision \newline
3. Update dinner time &
Verify: \newline
- Safety maintained \newline
- Dependencies satisfied \\
\hline
\end{tabular}
\label{tab:adjustments}
\end{table*}

==> MACIAgents.tex <==
To address these limitations, we propose Multi-Agent Collaborative Intelligence (MACI), a framework comprising specialized agents to improve planning effectiveness.
We illustrate its application to travel planning, utilizing several 
helpful agents organized into three categories, meta-planning agents,
support and validation agents, specialized enhance agents.

\paragraph{Primary Planning Agents}
\begin{enumerate}
   \item \textbf{Common Sense Interpretation Agent}: Identifies implicit constraints and practical considerations by:
       \begin{itemize}
           \item Analyzing task requirements for unstated assumptions
           \item Incorporating real-world knowledge into planning
           \item Flagging potential practical obstacles
       \end{itemize}
   
   \item \textbf{Social Interpretation Agent}: Manages human-centric aspects by:
       \begin{itemize}
           \item Understanding interpersonal dependencies
           \item Considering individual preferences and limitations
           \item Evaluating social feasibility of plans
       \end{itemize}
   
   \item \textbf{Spatial Constraint Analysis Agent}: Handles spatial relationships through:
       \begin{itemize}
           \item Geographic dependency modeling
           \item Travel time estimation
           \item Location-based constraint management
       \end{itemize}
   
   \item \textbf{Temporal Constraint Analysis Agent}: Manages time-based constraints via:
       \begin{itemize}
           \item Schedule optimization
           \item Temporal dependency tracking
           \item Deadline management
       \end{itemize}
\end{enumerate}

\paragraph{Support and Validation Agents}
\begin{enumerate}[resume]
   \item \textbf{Constraint Validation Agent}: Ensures plan validity through:
       \begin{itemize}
           \item Cross-constraint verification
           \item Consistency checking
           \item Violation detection
       \end{itemize}
   
   \item \textbf{Collaborative Reasoning Agent}: Coordinates multi-agent insights by:
       \begin{itemize}
           \item Integrating agent perspectives
           \item Resolving conflicts
           \item Maintaining global coherence
       \end{itemize}
\end{enumerate}

\paragraph{Specialized Enhancement Agents}
\begin{enumerate}[resume]
   \item \textbf{Resource Management Agent}: Optimizes resource allocation through:
       \begin{itemize}
           \item Inventory tracking
           \item Capacity planning
           \item Utilization optimization
       \end{itemize}
   
   \item \textbf{Safety Monitor Agent}: Ensures critical safety constraints by:
       \begin{itemize}
           \item Risk assessment
           \item Safety rule enforcement
           \item Emergency protocol management
       \end{itemize}
   
   \item \textbf{Optimization Agent}: Improves plan quality through:
       \begin{itemize}
           \item Efficiency analysis
           \item Alternative path exploration
           \item Continuous refinement
       \end{itemize}
\end{enumerate}


==> MACIExpOLD.tex <==
\section{Evaluating $\mathcal{MP}$'s Planning Capabilities}
\label{sec:MACIExp}

We evaluate the meta-planner $\mathcal{MP}$ through two experiments. First, we revisit the Thanksgiving dinner planning scenario that revealed limitations in single-LLM approaches. Second, we evaluate $\mathcal{MP}$ using IPC-2023 (International Planning Competition) benchmarks \cite{vallati2023temporal}, comparing its performance against state-of-the-art planning systems.

\subsection{Thanksgiving Dinner Planning}

The problem statement remains consistent with Section~\ref{sec:MACIcasestudy}, with $\mathbf{W^*}$ 
generated by $\mathcal{MP}$ to enhance constraints and dependencies. Planning performance is compared across four configurations: DeepSeek, GPT4o, DeepSeek + $\mathcal{MP}$, and GPT4o + $\mathcal{MP}$.

As demonstrated in Section~\ref{sec:MACIcasestudy}, both DeepSeek and GPT4o failed to satisfy the constraints. Therefore, we focus on comparing DeepSeek + $\mathcal{MP}$ and GPT4o + $\mathcal{MP}$ using the following metrics:
\vspace{-.15in}
\[
\text{Performance} = \{\% \text{constraint satisfaction, flexibility}\},
\vspace{-.15in}
\]

where flexibility is measured by the proactively incorporated slack time in the plan to handle unexpected surprises.

\subsubsection{Meta-Planning for Thanksgiving Event}

Following \textbf{Algorithm} 1, $\mathcal{MP}$ generates a  workflow for the Thanksgiving dinner planning task. This workflow consists of role nodes (cook, drivers, supervisor), explicit constraint edges (temporal, spatial, resource), and additional implicit constraint edges identified through common-sense analysis. The complete planner includes agent specifications for both node and edge monitoring, along with protocols for dynamic adjustments and validation. The complete planner specification, including detailed agent protocols and adjustment procedures, is provided in Appendix~\ref{app:MACIExpDetails}.


%The workflow implements four key monitoring categories:
%\begin{itemize}[leftmargin=1.5em, topsep=-.15em, parsep=-.15em]
%\item Role assignment and qualification verification
%\item Temporal and spatial dependency tracking
%\item Resource allocation and constraint management
%\item Safety and supervision monitoring
%\end{itemize}


{\color{red}{Completed up to here, working on Appendices now.}}
\subsubsection{Plan Execution and Verification}

\textbf{Error Analysis in Initial Plan}

Let me revise the schedule with corrected timing:

\begin{table*}[ht]
\caption{Corrected Dynamic Adjustment Plan: James's 3-Hour Flight Delay}
\small
\begin{tabular}{|p{0.12\textwidth}|p{0.28\textwidth}|p{0.28\textwidth}|p{0.22\textwidth}|}
\hline
\textbf{Time} & \textbf{Event} & \textbf{Action} & \textbf{Constraints} \\
\hline
2:00 PM & Turkey Start & Sarah puts turkey in oven & Must be watched for 4 hours \\
\hline
2:30 PM & Emily Lands & Start 30-min luggage claim & Airport process time \\
\hline
3:00 PM & Michael Arrives Home & Available for pickup duty & Driver transition time \\
\hline
3:15 PM & Emily Ready & Michael departs for airport & After luggage claim \\
\hline
4:15 PM & Emily Returns Home & Can start side dishes & 2-hour prep needed \\
\hline
4:30 PM & Grandma Pickup & Sarah continues oven duty & Supervision maintained \\
\hline
6:15 PM & Dinner Served & Side dishes require full 2 hours & Delayed from original 6:00 PM \\
\hline
\end{tabular}
\end{table*}

The revised schedule accounts for:
- Correct luggage claim time
- Michael's actual arrival time
- Full 2-hour side dish preparation
- Continuous oven supervision

This delay necessitates pushing dinner to 6:15 PM.

\begin{table}[th]
\caption{A Schedule with Maximal Slack Time. Sarah is available to drive between 2:00 PM and 5:00 PM.}
%\vspace{-.1in}
\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|p{4cm}|l|}
\hline
\textbf{Time} & \textbf{Task} & \textbf{Assigned} \\
\toprule
\hline
1:00pm & Sarah picks up Grandma & Sarah \\
2:00pm & Sarah Grandma returns home  & - \\
2:00pm & Turkey in the oven & Sarah \\
2:00pm & Oven watch starts (fire hazard) & GM or Sarah \\
2:30pm & Emily arrives at BOS & - \\
3:00pm & Michael picks up Emily at BOS & Michael \\
4:00pm & James lands at BOS & James \\
4:00pm & Michael and Emily arrive home & - \\
4:30pm & Picks up rental car heads home & James \\
4:00pm & Side dish preparation begins & Everyone - J \\
5:30pm & James arrives home & - \\
6:00pm & Thanksgiving dinner served & Everyone \\
\hline
\end{tabular}
\end{center}
\label{tab:Retrospective}
\end{footnotesize}
\end{table}


\subsection{IPC-2023}

We evaluate MACI using IPC-2023 temporal planning benchmarks
\cite{vallati2023temporal}, focusing on logistics domains that require coordination of multiple activities with temporal constraints. These problems align with our Thanksgiving dinner scenario, involving resource allocation, temporal dependencies, and concurrent activity management.

Performance is measured against:
\begin{equation}
Score = \sum_{p \in P} \frac{T^*_p}{T_p}
\end{equation}
where $T^*_p$ is the best known makespan for problem $p$, and $T_p$ is our solution's makespan.

This direct comparison with current state-of-the-art temporal planners demonstrates that MACI achieves state-of-the-art results, surpassing all prior systems.

==> MACISpecOLD.tex <==
\section{MACI Framework Specification}
\label{sec:MACISpec}

MACI implements a three-layer architecture to address current LLM limitations: metacognitive constraints, attention bias, and gaps in common-sense reasoning. The top two layers represent key innovations, while the bottom layer leverages existing multi-agent system (MAS) infrastructure.

\subsection{Three-Layer Architecture}
\label{sec:MACI-threetiers}
%\vspace{-.1in}
\paragraph{Meta-Planner: The Planning Generator}
The meta-planner $\mathcal{MP}$ functions as a higher-order planner that generates task-specific planning systems:
\[
\mathcal{MP}: (\mathcal{O}, \mathcal{C_E}) \rightarrow \mathbf{W},
\]
where $\mathbf{W}$ represents a planning system composed of specialized, coordinated agents. Similar to how a compiler generator produces compilers from specifications, $\mathcal{MP}$ constructs agent networks from task requirements. It analyzes objectives, identifies required roles and dependencies, selects appropriate agents, and establishes interaction protocols. This produces a complete workflow template defining both the planning state space and the agent coordination mechanisms needed to solve the given task.

\vspace{-.1in}
\paragraph{Agent Repository Layer} 
This layer maintains a distributed collection of planning agents, each designed with a restricted context window and specialized interface. By dividing cognitive tasks among agents, this architecture ensures a complete knowledge of the constraints without overwhelming individual components.
\vspace{-.1in}
\paragraph{System Infrastructure Layer} 
Built on open-source MAS frameworks, the infrastructure layer supports essential operations such as agent registration, message routing, resource allocation, and deployment scaling.

\subsection{Agent Repository Layer Design}

\subsubsection{Agent Registration and Search Protocol}
Agents register in the repository with five attributes: input/output protocol ($P$), type ($t$), capability vector ($c$), context window size ($w \leq 1k$ tokens) and user rating ($r$). These attributes enable $\mathcal{MP}$  to match task requirements to agent capabilities efficiently. $\mathcal{MP}$ searches for agents by:
1) matching task requirements to capability descriptions ($c$),
2) filtering by agent type ($t$) and user ratings ($r$),
and 3) verifying protocol compatibility ($P$).

\subsubsection{State Space and Agent Design}


\paragraph{General State Space}

%- \emph{Who} tracks actors, their roles, and role constraints.
%- \emph{Where} represents physical and logical locations.
%- \emph{When} captures temporal constraints, including deadlines and durations.
%- \emph{What} describes resources, their constraints, and associated costs.
%- \emph{Why} tracks rationale and dependencies, enabling reasoning about decision-making.

\begin{table}[th!]
%\vspace{-.2in}
\caption{State Space Dimensions and Components}
\begin{footnotesize}
\begin{tabular}{|p{0.08\textwidth}|p{0.14\textwidth}|p{0.18\textwidth}|}
\hline
\textbf{Dimension} & \textbf{Core Components} & \textbf{Example States} \\
\toprule
\hline
Who \newline (Actors) & • Actor ID \newline • Current Roles \newline • Role Constraints \newline • Role Changes & • Driver vs Passenger \newline • Supervisor vs Worker \newline • Buyer vs Seller \newline • Multiple role conflicts \\
\hline
Where \newline (Location) & • Current Position \newline • Target Location \newline • Transition Points \newline • Access Rules & • Physical locations \newline • Virtual positions \newline • State transitions \newline • Boundary constraints \\
\hline
When \newline (Time) & • Time Points \newline • Duration \newline • Deadlines \newline • Probability & • Event timestamps \newline • Process duration \newline • Completion times \newline • Delay likelihood \\
\hline
What \newline (Resources) & • Methods \newline • Requirements \newline • Constraints \newline • Costs & • Tools/Vehicles \newline • Tickets/Permits \newline • Capacity limits \newline • Time-money trade-offs \\
\hline
Why \newline (Logic) & • Rationale \newline • Dependencies \newline • Risks \newline • Alternatives & • Decision basis \newline • Causal chains \newline • Failure modes \newline • Backup plans \\
\hline
\end{tabular}
\end{footnotesize}
\label{tab:state_space}
\vspace{-.1in}
\end{table}


Table~\ref{tab:state_space} presents five dimensions of state space, Who, Where, When, What, and Why, that form the basis of planning tasks. These dimensions are general enough to apply across domains, with travel planning serving as an illustrative example. 
\vspace{-.1in}
\paragraph{Common Agents}
Common agents are designed to handle core planning and validation tasks that are universally applicable across domains. These agents provide foundational capabilities that ensure the consistency, feasibility, and robustness of planning systems, regardless of the specific application. Their roles align with the general state space dimensions of \emph{Who, Where, When, What,} and \emph{Why}, ensuring that all essential aspects of planning are addressed.
For a list of common agents, please refer to 
Appendix~\ref{app:ExampleCommonAgents}.

These agents work collaboratively to ensure robust planning and validation across diverse domains. Although the list of common agents is not exhaustive, it provides a strong foundation to address most planning tasks. New common agents can be introduced as the need arises, provided they offer capabilities that can be reused across multiple domains. For example, an \emph{Adaptation Agent} could be added to dynamically adjust constraints in response to evolving task environments.

\vspace{-.1in}
\paragraph{Specialized Agents}
Specialized agents extend the capabilities of MACI by addressing domain-specific requirements that are not generalizable across all tasks. These agents are designed to implement detailed knowledge and expertise tailored to specific applications, ensuring that MACI remains adaptable and effective for diverse planning challenges. Specialized agents typically focus on tasks requiring unique constraint handling, optimization, or analysis.

Examples of specialized agents include the following.
\begin{itemize}[leftmargin=1.2em, topsep=-.15em, parsep=-.15em]
    \item \emph{Travel Planning Agent}: Optimizes itineraries, manages transportation options, and ensures seamless transitions between locations.
    \item \emph{Financial Risk Agent}: Monitors market trends, assesses risks, and validates investment strategies.
    \item \emph{Healthcare Resource Agent}: Allocates medical supplies, schedules staff, and optimizes patient care pathways.
    \item \emph{Supply Chain Agent}: Manages logistics, tracks inventory, and optimizes distribution routes.
\end{itemize}

Specialized agents adhere to architectural principles that maintain consistency and integration within MACI:
\begin{itemize}[leftmargin=1.2em, topsep=-.15em, parsep=-.15em]
    \item \emph{Restricted Context Windows}: Each agent operates within a limited context to ensure efficiency and focus ($w \leq 1k$ tokens).
    \item \emph{Protocol Buffer Interfaces}: Standardized interfaces enable seamless communication between agents.
    \item \emph{Coordination with Common Agents}: Specialized agents leverage the capabilities of common agents for validation, compliance, and constraint management.
    \item \emph{Domain-Specific Constraints}: Specialized agents are equipped to handle unique requirements and challenges specific to their domain.
\end{itemize}


%%%%%%%%%%%
\begin{comment}
\paragraph{Generalization and Domain Adaptation}
While common agents provide broad capabilities, specialized agents ensure MACI’s adaptability to diverse applications. The travel planning example illustrates how specialized agents interact with common agents to create effective and robust plans. For example, the Temporal Agent validates flight schedules, while the Travel Planning Agent optimizes transitions between locations. This modular approach enables cross-domain generalization, where new domains can reuse existing common agents while introducing tailored specialized agents. Future work will focus on expanding this library of agents and developing mechanisms to streamline the integration of new domain-specific agents into the MACI framework.

\paragraph{Illustrative Example in Travel Planning}
In travel planning, actors (\emph{Who}) transition between roles, such as drivers or passengers, each with specific constraints. Locations (\emph{Where}) represent destinations and waypoints, while temporal constraints (\emph{When}) include schedules and deadlines. Resources (\emph{What}) like vehicles or tickets are managed to meet cost and capacity constraints, and the rationale (\emph{Why}) links these decisions to objectives. This example demonstrates MACI functionality, but is not exhaustive; the following sections address how MACI is generalized across domains.
\end{comment}
%%%%%%%%%%

\subsubsection{Agent Coordination and State \& Constraint Management}
MACI ensures seamless coordination between agents across state dimensions. For example, in travel planning, when a Schedule Agent detects a flight connection constraint, it triggers updates to Location, Resource, and Role Manager Agents. These updates propagate through a state transition protocol, where the proposed state change is validated against global and local constraints:
\vspace{-.05in}
\[
T: S_t \rightarrow S_{t+1} \text{ subject to } C_{\text{global}} \land C_{\text{local}}
\]
\vspace{-.25in}

\subsubsection{Validation Protocols}

The validation agent ensures state consistency by decomposing global constraints into dimension-specific checks. For example, when booking a flight, the temporal agent validates the temporal constraint, the spatial feasibility is checked by the location agent, and the availability of seats is validated by the resource agent. Common sense agents identify overlooked constraints, such as luggage claiming time, inter-terminal walking time, and rental car pickup time. If validation fails, the system triggers a recovery process to generate alternative solutions. Validation protocols can be updated when unexpected events occur to improve retrospective planning. 

%The validation protocols described above align closely with established methods in operations research (OR). Please refer to Appendix~\ref{app:MACIValidationRecovery} for a detailed discussion of the protocols.

\subsubsection{Other Considerations}

Due to space limitation, we document in
Appendix~\ref{app:MACIMore} additional considerations including
cross-domain generalization, enhancement and integration of common sense knowledge, scalability, and a list of future enhancements when more applications
will be supported.

\subsection{Meta-Planner: Planning a Planner to Plan}

The meta-planner $\mathcal{MP}$  operates as a higher-level planner that constructs other planners, which are actionable workflows for specific tasks. 

\subsubsection{The Meta-Planner Algorithm}

$\mathcal{MP}$ is specified in \textbf{Algorithm} \#1.  A list of all symbols used in the specifications is provided in Table~\ref{tab:MACIsymbols} in Appendix~\ref{app:MACITF}.

A workflow network $\mathbf{W} = (\mathcal{N}, \mathcal{E})$, represented as a directed graph, consists of roles as nodes and their dependencies as edges. The nodes $n \in \mathcal{N}$ denote the roles performed by human actors (e.g. driver, cook, supervisor), while the edges $e_{ij} \in \mathcal{E}$ between the nodes $n_i$ and $n_j $ capture the monitored dependencies (e.g., temporal, spatial constraints, data dependencies and safety requirements for supervision).

\vspace{-.1in}
\begin{equation}
\mathbf{W} = (\mathcal{N}, \mathcal{E}), \text{ where } \mathcal{N} = A^*_n \text{ and } \mathcal{E}  = A^*_e.
\vspace{-.1in}
\label{eq:MACIObjective}
\end{equation}

\begin{algorithm}[th!]
\caption{$\mathcal{MP}$: Planner for Planning a Plan}
\begin{algorithmic}
\INPUT Objectives $\mathcal{O}$, explicit constraints $\mathcal{C_E}$, agent pool $\mathbf{A}$, people $\mathcal{P}$, metrics $\mathcal{M}$
\OUTPUT Optimized workflow $\mathbf{W^*} = (\mathcal{N}, \mathcal{E})$ \hfill (\textbf{Eq}. \ref{eq:MACIObjective})
\STATE // Phase 1: Network Construction
\STATE 1. $\mathcal{N}$: Extract roles \& capabilities from $\mathcal{O}$ \hfill (\textbf{Eq}. \ref{eq:roleq})
\STATE 2. $\mathcal{E}$: Identify node dependencies from $\mathcal{C_E}$ \hfill (\textbf{Eq}. \ref{eq:constraintq})
\STATE // Phase 2: Agent Assignment
\STATE 3. Assign role agents: $\forall n \in \mathcal{N}$, select $\alpha_n \in \mathbf{A_n}$ \hfill (\textbf{Eq}. \ref{eq:nodeagentq})
\STATE 4. Assign edge agents: $\forall e_{ij} \in \mathcal{E}$, $\alpha_{ij} \in \mathbf{A_e}$ \hfill (\textbf{Eq}. \ref{eq:edgeagentq})

\STATE // Phase 3: Iterative Refinement
\WHILE{improvement in $V(\mathbf{W}, \mathcal{M})$}
   \STATE // Role Assignment Optimization
   \FORALL{$n \in \mathcal{N}$}
       \STATE Update role-person mappings via $f_{\text{role}}(n, \mathcal{P})$
   \ENDFOR
   
   \STATE // Dependency Monitoring
   \FORALL{$e \in \mathcal{E}$}
       \STATE Verify dependencies via assigned edge agents
   \ENDFOR
   
   \STATE // Validation
   \IF{$V(\mathbf{W_{new}}, \mathcal{M}) > V(\mathbf{W_{current}}, \mathcal{M})$}
       \STATE $\mathbf{W_{current}} \gets \mathbf{W_{new}}$
   \ENDIF
\ENDWHILE
\STATE \textbf{return} $\mathbf{W^*} = \mathbf{W{current}}$
\end{algorithmic}
\end{algorithm}

$\mathcal{MP}$  constructs a planner in three phases. First, it builds the network structure by identifying roles and their dependencies, forming the foundation of the workflow.

Second, it assigns appropriate agents to manage both roles and dependencies. Each node \(n \in \mathcal{N}\) is managed by a designated role agent \(\alpha_{n}\). Similarly, each edge \(e_{ij} \in \mathcal{E}\), representing a dependency between nodes, is managed by an agent \(\alpha_{ij}\), which connects the node agents \(\alpha_i\) and \(\alpha_j\). These edges are enriched with metadata that may include details such as data types, communication protocols, timing constraints, and security requirements.

Finally, the generated planner iteratively refines the workflow. This process involves optimizing role assignments and continuously monitoring dependencies until the validation score stabilizes, ensuring a well-validated workflow.

\subsubsection{Meta-Planning Components}

Let us clearly distinguish between roles (requiring human qualifications) and monitoring tasks (requiring capabilities).

\paragraph{Role and Qualification Analysis}
$\mathcal{MP}$ analyzes objectives $\mathcal{O}$ to identify required roles and their qualifications:
\begin{equation}
\text{map}_{\text{role}}: \mathcal{O} \rightarrow \{(n_i, q_i)\}
\label{eq:roleq}
\end{equation}
where $n_i$ represents a role and $q_i$ its required qualifications. For example, $(n_{\text{driver}}, q_{\text{license}})$ or $(n_{\text{cook}}, q_{\text{experience}})$.

\paragraph{Constraint Management}
The framework maintains a global constraint set $C$ composed of:
\begin{equation}
C = C_{E} \cup C_I \cup C_D
\label{eq:constraintq}
\end{equation}
where $C_{E}$ represents explicit constraints from problem specification, $C_I$ denotes implicit constraints identified by Common Sense Agent, and $C_D$ represents derived constraints from agent interactions.


\paragraph{Agent Assignment}
Two types of agents, node and edge, are selected from the repository $\mathbf{A}$:

1. Node Monitoring Agents:
\begin{equation}
%\text{select}_{\text{node}}: 
A^*_n = \argmin_{A_i \in \mathbf{A}} \sum_{n_j} \text{dist}(q_j, A_i.\text{capabilities})
\label{eq:nodeagentq}
\end{equation}
These agents verify role qualifications and manage people-role assignments and transitions.

2. Edge Monitoring Agents:
\begin{equation}
%\text{select}_{\text{edge}}: 
A^*_e = \argmin_{A_i \in \mathbf{A}} \sum_{e_j} \text{dist}(c_j, A_i.\text{capabilities})
\label{eq:edgeagentq}
\end{equation}
These agents monitor dependencies between roles, where $c_j$ represents constraint types (temporal, spatial, etc.).

$\mathcal{MP}$ iteratively refines the network by validating workflow constraints and performance and replacing or adding agents, i.e., checking and adding nodes and edges.

\subsection{Workflow Execution Framework}

The workflow $\mathbf{W^*}$ requires a runtime system for execution. In this work, we evaluate $\mathbf{W^*}$ by entering $\mathbf{W^*}$ along with the problem statement into an LLM (DeepSeek and GPT4o). A key limitation is that the feedback loop for refining $\mathbf{W^*}$ must be performed manually.


==> PlanningTypes.tex <==
\paragraph{Planning Types}
Planning can be classified into seven types.
The first three are considered more strategic and the rest are
tactic methodologies. 

\vspace{-0.2em}
\begin{enumerate}[leftmargin=1.5em, topsep=-.1em, parsep=-.1em]
\item \textit{Sequential planning}: Creates time-ordered schedules meeting goals/constraints via formal temporal representations \cite{allen1989moments}
\item \textit{Proactive planning}: Anticipates future scenarios to preemptively address issues through deliberate foresight \cite{cox1998goal} 
\item \textit{Retrospective planning}: Improves future plans by analyzing past experiences via case-based reasoning \cite{kolodner1993case}
\item \textit{Adaptive planning}: Adjusts plans to changing conditions while preserving core constraints \cite{hammond1990case}
\item \textit{Reactive planning}: Prioritizes immediate actions over long-term goals in dynamic, uncertain environments \cite{georgeff1987reactive}
\item \textit{Predictive planning}: Uses data-driven models to forecast scenarios and optimize decisions \cite{kushmerick1995algorithm}
\end{enumerate}

\vspace{-0.5em}
\begin{comment}
    

\begin{enumerate}[leftmargin=1.5em, topsep=-.1em, parsep=-.1em]
\item \textit{Sequential planning} establishes the foundational schedule that satisfies the goals and constraints in a specific time order. According to Allen and Hayes \cite{allen1989moments}, this requires the formal representation of temporal information and relationships to establish viable action sequences.

\item \textit{Proactive planning} anticipates potential future scenarios and prepares contingencies before they occur. Cox and Veloso \cite{cox1998goal} describe this as deliberately reasoning about future states to prevent problems rather than solving them after they arise.

\item \textit{Retrospective planning} examines completed experiences to improve future planning effectiveness. Kolodner \cite{kolodner1993case} describes this as a case-based reasoning approach where past experiences inform and enhance future planning capabilities.

\item \textit{Adaptive planning} modifies existing plans in response to changing circumstances while maintaining critical constraints. As defined by Hammond \cite{hammond1990case}, it involves plan modification strategies that preserve plan coherence while accommodating new situations or information.

\item \textit{Reactive planning} handles immediate situations that require quick decisions without complete information. According to \cite{georgeff1987reactive}, reactive planning differs from traditional planning by focusing on immediate action selection rather than long-term goal achievement.

\item \textit{Predictive planning} employs data analysis and pattern recognition to predict likely scenarios and inform planning decisions. As outlined by Kushmerick et al. \cite{kushmerick1995algorithm}, this involves using learned models to predict outcomes and guide planning choices.
\end{enumerate}
\end{comment}
